Towards Reasonably-Sized Character-Level Transformer NMT by Finetuning Subword Systems

Applying the Transformer architecture on the character level usually requires very deep architectures that are difficult and slow to train. These problems can be partially overcome by incorporating a segmentation into tokens in the model. We show that by initially training a subword model and then finetuning it on characters, we can obtain a neural machine translation model that works at the character level without requiring token segmentation. We use only the vanilla 6-layer Transformer Base architecture. Our character-level models better capture morphological phenomena and show more robustness to noise at the expense of somewhat worse overall translation quality. Our study is a significant step towards high-performance and easy to train character-based models that are not extremely large.

==> table.tex <==
\newcommand\cellScaleColor[2]
  {\colorbox{GreenYellow!#1}{#2}}
  %{\colorbox{yellow!#1!green}{#2}}

\newcommand{\Bende}[1]{%
	\pgfmathsetmacro{\Min}{22.57}
	\pgfmathsetmacro{\Max}{26.86}
	\pgfmathsetmacro{\PercentColor}{max(min(100.0 * (#1 - \Min)/(\Max - \Min), 100.0), 0.00)} %
    \hspace{-0.33em}\cellScaleColor{\PercentColor}{#1}
}
\newcommand{\Cende}[1]{%
	\pgfmathsetmacro{\Min}{0.5262}
	\pgfmathsetmacro{\Max}{0.5692}
	\pgfmathsetmacro{\PercentColor}{max(min(100.0 * (#1 - \Min)/(\Max - \Min), 100.0), 0.00)} %
	\hspace{-0.33em}\cellScaleColor{\PercentColor}{#1}
}
\newcommand{\Mende}[1]{%
	\pgfmathsetmacro{\Min}{45.00}
	\pgfmathsetmacro{\Max}{47.95}
	\pgfmathsetmacro{\PercentColor}{max(min(100.0 * (#1 - \Min)/(\Max - \Min), 100.0), 0.00)} %
	\hspace{-0.33em}\cellScaleColor{\PercentColor}{#1}
}
\newcommand{\Nende}[1]{%
	\pgfmathsetmacro{\Min}{-1.075}
	\pgfmathsetmacro{\Max}{-0.990}
	\pgfmathsetmacro{\PercentColor}{max(min(100.0 * (#1 - \Min)/(\Max - \Min), 100.0), 0.00)} %
	\hspace{-0.33em}\cellScaleColor{\PercentColor}{#1}
}

\newcommand{\Rende}[1]{%
	\pgfmathsetmacro{\Min}{89.18}
	\pgfmathsetmacro{\Max}{90.10}
	\pgfmathsetmacro{\PercentColor}{max(min(100.0 * (#1 - \Min)/(\Max - \Min), 100.0), 0.00)} %
	\hspace{-0.33em}\cellScaleColor{\PercentColor}{#1}
}

\newcommand{\Bdeen}[1]{%
	\pgfmathsetmacro{\Min}{26.62}
	\pgfmathsetmacro{\Max}{30.14}
	\pgfmathsetmacro{\PercentColor}{max(min(100.0 * (#1 - \Min)/(\Max - \Min), 100.0), 0.00)} %
    \hspace{-0.33em}\cellScaleColor{\PercentColor}{#1}
}

\newcommand{\Cdeen}[1]{%
	\pgfmathsetmacro{\Min}{.5433}
	\pgfmathsetmacro{\Max}{.5732}
	\pgfmathsetmacro{\PercentColor}{max(min(100.0 * (#1 - \Min)/(\Max - \Min), 100.0), 0.00)} %
    \hspace{-0.33em}\cellScaleColor{\PercentColor}{#1}
}

\newcommand{\Mdeen}[1]{%
	\pgfmathsetmacro{\Min}{35.07}
	\pgfmathsetmacro{\Max}{37.42}
	\pgfmathsetmacro{\PercentColor}{max(min(100.0 * (#1 - \Min)/(\Max - \Min), 100.0), 0.00)} %
    \hspace{-0.33em}\cellScaleColor{\PercentColor}{#1}
}

\newcommand{\Ndeen}[1]{%
	\pgfmathsetmacro{\Min}{-0.451}
	\pgfmathsetmacro{\Max}{-0.364}
	\pgfmathsetmacro{\PercentColor}{max(min(100.0 * (#1 - \Min)/(\Max - \Min), 100.0), 0.00)} %
    \hspace{-0.33em}\cellScaleColor{\PercentColor}{#1}
}

\newcommand{\Bencs}[1]{%
	\pgfmathsetmacro{\Min}{18.24}
	\pgfmathsetmacro{\Max}{21.07}
	\pgfmathsetmacro{\PercentColor}{max(min(100.0 * (#1 - \Min)/(\Max - \Min), 100.0), 0.00)} %
    \hspace{-0.33em}\cellScaleColor{\PercentColor}{#1}
}

\newcommand{\Cencs}[1]{%
	\pgfmathsetmacro{\Min}{0.4645}
	\pgfmathsetmacro{\Max}{0.4899}
	\pgfmathsetmacro{\PercentColor}{max(min(100.0 * (#1 - \Min)/(\Max - \Min), 100.0), 0.00)} %
    \hspace{-0.33em}\cellScaleColor{\PercentColor}{#1}
}

\newcommand{\Mencs}[1]{%
	\pgfmathsetmacro{\Min}{24.57}
	\pgfmathsetmacro{\Max}{25.98}
	\pgfmathsetmacro{\PercentColor}{max(min(100.0 * (#1 - \Min)/(\Max - \Min), 100.0), 0.00)} %
    \hspace{-0.33em}\cellScaleColor{\PercentColor}{#1}
}

\newcommand{\Nencs}[1]{%
	\pgfmathsetmacro{\Min}{-1.032}
	\pgfmathsetmacro{\Max}{-0.816}
	\pgfmathsetmacro{\PercentColor}{max(min(100.0 * (#1 - \Min)/(\Max - \Min), 100.0), 0.00)} %
    \hspace{-0.33em}\cellScaleColor{\PercentColor}{#1}
}

\newcommand{\Rencs}[1]{%
	\pgfmathsetmacro{\Min}{81.28}
	\pgfmathsetmacro{\Max}{84.87}
	\pgfmathsetmacro{\PercentColor}{max(min(100.0 * (#1 - \Min)/(\Max - \Min), 100.0), 0.00)} %
    \hspace{-0.33em}\cellScaleColor{\PercentColor}{#1}
}

\newcommand{\Tencs}[1]{%
	\pgfmathsetmacro{\Min}{4.48}
	\pgfmathsetmacro{\Max}{5.84}
	\pgfmathsetmacro{\PercentColor}{max(min(100.0 * (#1 - \Min)/(\Max - \Min), 100.0), 0.00)} %
    \hspace{-0.33em}\cellScaleColor{\PercentColor}{#1}
}

\newcommand{\Bentr}[1]{%
	\pgfmathsetmacro{\Min}{11.55}
	\pgfmathsetmacro{\Max}{13.11}
	\pgfmathsetmacro{\PercentColor}{max(min(100.0 * (#1 - \Min)/(\Max - \Min), 100.0), 0.00)} %
    \hspace{-0.33em}\cellScaleColor{\PercentColor}{#1}
}

\newcommand{\Centr}[1]{%
	\pgfmathsetmacro{\Min}{0.4500}
	\pgfmathsetmacro{\Max}{0.4620}
	\pgfmathsetmacro{\PercentColor}{max(min(100.0 * (#1 - \Min)/(\Max - \Min), 100.0), 0.00)} %
    \hspace{-0.33em}\cellScaleColor{\PercentColor}{#1}
}

\newcommand{\Nentr}[1]{%
    \pgfmathsetmacro{\Min}{-0.916}
	\pgfmathsetmacro{\Max}{-0.657}
	\pgfmathsetmacro{\PercentColor}{max(min(100.0 * (#1 - \Min)/(\Max - \Min), 100.0), 0.00)} %
    \hspace{-0.33em}\cellScaleColor{\PercentColor}{#1}
}

\newcommand\compare[2]{%
    \scriptsize \IfSubStr{#1}{-}{\color{BrickRed} #1}{\color{ForestGreen} #1} \color{black} {\tiny /} \IfSubStr{#2}{-}{\color{BrickRed} #2}{\color{ForestGreen} #2}
}
\newcommand\fromBest[1]{\scriptsize \textcolor{BrickRed}{#1}}
\newcommand\best{\scriptsize $\ast$}

\newcolumntype{C}{>{\centering\arraybackslash}p{1.08cm}}


\adjustbox{max width=\textwidth}{%
\begin{tabular}{ll|CCCCCCCC|ccc|c}
\toprule

& & \multicolumn{8}{c|}{From random initialization}
& \multicolumn{3}{c|}{Direct finetuning from}
%& \multicolumn{5}{c}{Curriculum: 500 $\rightarrow$ \ldots} \\
& \multirow{2}{*}{In steps} \\

\cmidrule(lr){3-10} \cmidrule(lr){11-13} %\cmidrule(lr){13-17}

% From ranom initialization
& & 32k & 16k & 8k & 4k & 2k & 1k & 500 & 0 &
% Direct finetuning
500 & 1k & 2k & % 16k &
% Complete curriculum
%250 & 150 & 100 & 50 & 0 \\ \midrule
\\ \midrule



% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%   ENGLISH -> GERMAN
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\multirow{6}{*}{\rotatebox{90}{en-de}}
& \multirow{2}{*}{BLEU} &
    % From random initialization
    \Bende{26.85} & \Bende{26.86} & \Bende{26.66} & \Bende{26.39} & \Bende{26.36} & \Bende{26.08} & \Bende{25.79} & \Bende{22.57} &
    % Direct finetuning
    \Bende{25.21} & \Bende{24.98} & \Bende{25.01} & % \Bende{23.43} &
    % Complete curriculum
    % \Bende{25.28} & \Bende{25.00} & \Bende{24.87} & \Bende{24.83} & \Bende{24.45}
    % Final curriculum
    \Bende{24.63}

\\

   &  &  % Comparing BLEU to the best scores
    % From random initialization
    \fromBest{-0.03} & \best & \fromBest{-0.20} & \fromBest{-0.47} & \fromBest{-0.50} & \fromBest{-0.78} & \fromBest{-1.07} & \fromBest{-4.29} &
    % Direct finetuning
    \compare{-1.65}{-0.58} & \compare{-1.88}{-1.10} & \compare{-1.85}{-0.78} &
    % Final curriculum
    \compare{-2.23}{-1.16}
\\
& chrF &
    % From random initialization
    \Cende{.5692} & \Cende{.5675} & \Cende{.5677} & \Cende{.5680} & \Cende{.5644} & \Cende{.5642} & \Cende{.5612} & \Cende{.5262} &
    % Direct finetuning
    \Cende{.5588} & \Cende{.5596} & \Cende{.5593} & % \Cende{.5456} &
    % Complete curriculum
    %\Cende{.5585} & \Cende{.5563} & \Cende{.5550} & \Cende{.5545} & \Cende{.5545}
    % Final curriculum
    \Cende{.5559}
\\

%   &  &  % Comparing CHRF to the best scores
%    % From random initialization
%   \fromBest{\ast} & \fromBest{-.0017} & \fromBest{-.0019} & \fromBest{-.0012} & \fromBest{-.0048} & \fromBest{-.0050} & \fromBest{-.0080} &
%    % Direct finetuning
%    \compare{-1.65}{-0.58} & \compare{-1.88}{-1.10} & \compare{-1.85}{-0.78} &
%    % Final curriculum
%    \compare{-2.23}{-1.16}
%
%    \\

& METEOR &
    % From random initialization
    \Mende{47.68} & \Mende{47.95} & \Mende{47.89} & \Mende{47.75} & \Mende{47.91} & \Mende{47.71} & \Mende{47.58} & \Mende{45.00} &
    % Direct finetuning
    \Mende{46.52} & \Mende{46.37} & \Mende{46.37} & % \Mende{45.09} &
    % Complete curriculum
    % \Mende{46.86} & \Mende{46.65} & \Mende{46.40} & \Mende{46.30} & \Mende{45.98}
    % Final curriculum
    \Mende{46.31}

\\ \cdashlinelr{2-14}

& Noise sens. &
    % From random initialization
    \Nende{-1.074} & \Nende{-1.062} & \Nende{-1.051} & \Nende{-1.032} & \Nende{-1.016} & \Nende{-1.021} & \Nende{-1.000} & \Nende{-0.846} &
    % Direct finetuning
    \Nende{-0.995} & \Nende{-0.990} & \Nende{-0.993} &
    % Complete curriculum
    %\Nende{-.2317} & \Nende{-.2247} & ? & ? & ?
    % Final curriculum
    \Nende{-0.876}
\\

& MorphEval &
    % From random initialization
    \Rende{89.97} & \Rende{89.52} & \Rende{89.41} &  \Rende{89.63} &  \Rende{89.77} &  \Rende{89.96} &  \Rende{89.19} & \Rende{89.16} &
    % Direct finetuning
    \Rende{89.88} & \Rende{90.29} & \Rende{89.97} &
    % Complete curriculum
    %\Rende{74.72} & \Rende{75.94} & \Rende{75.79} & \Rende{76.03} & \Rende{77.76}
    % Final curriculum
    \Rende{90.06}

\\ \midrule

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%   GERMAN -> ENGLISH
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\multirow{5}{*}{\rotatebox{90}{de-en}}
& \multirow{2}{*}{BLEU} &
    % From random initialization
    \Bdeen{29.79} & \Bdeen{30.13} & \Bdeen{29.60} & \Bdeen{29.26} & \Bdeen{28.61} & \Bdeen{28.46} & \Bdeen{28.14} & \Bdeen{26.62} &
    % Direct finetuning
    \Bdeen{28.19} & \Bdeen{28.36} & \Bdeen{27.71} & % \Bdeen{27.08} &
    % Complete curriculum
    %\Bdeen{28.53} & \Bdeen{28.26} & \Bdeen{28.10} & \Bdeen{27.91} & \Bdeen{27.91}
    % Final curriculum
    \Bdeen{28.24}
\\

   &  &  % Comparing BLEU to the best scores
    % From random initialization
   \fromBest{-0.34} & \best & \fromBest{-0.53} & \fromBest{-0.83} & \fromBest{-1.62} & \fromBest{-1.67} & \fromBest{-1.99} & \fromBest{-3.51} &
    % Direct finetuning
    \compare{-1.94}{+0.05} & \compare{-1.76}{-0.10} & \compare{-2.52}{-0.90} &
    % Final curriculum
    \compare{-1.89}{+0.10}
\\
& chrF &
    % From random initialization
    \Cdeen{.5701} & \Cdeen{.5732} & \Cdeen{.5681} & \Cdeen{.5670} & \Cdeen{.5619} & \Cdeen{.5582} & \Cdeen{.5577} & \Cdeen{.5433} &
    % Direct finetuning
    \Cdeen{.5618} & \Cdeen{.5641} & \Cdeen{.5586} & % \Cdeen{.5518} &
    % Complete curriculum
    %\Cdeen{.5634} & \Cdeen{.5617} & \Cdeen{.5617} & \Cdeen{.5603} & \Cdeen{.5601}
    % Final curriculum
    \Cdeen{.5625}
\\
& METEOR &
    % From random initialization
    \Mdeen{37.07} & \Mdeen{37.41} & \Mdeen{37.22} & \Mdeen{37.22} & \Mdeen{36.92} & \Mdeen{37.15} & \Mdeen{36.86} & \Mdeen{35.07} &
    % Direct finetuning
    \Mdeen{36.43} & \Mdeen{36.36} & \Mdeen{35.98} & % \Mdeen{35.51} &
    % Complete curriculum
    %\Mdeen{36.61} & \Mdeen{36.49} & \Mdeen{36.35} & \Mdeen{36.30} & \Mdeen{36.28}
    % Final curriculum
    \Mdeen{36.39}

\\ \cdashlinelr{2-14}

& Noise sens.&
    % From random initialization
    \Ndeen{-0.450} & \Ndeen{-0.435} & \Ndeen{-0.412} & \Ndeen{-0.423} & \Ndeen{-0.427} & \Ndeen{-0.417} & \Ndeen{-0.412} & \Ndeen{-0.303} &
    % Direct finetuning
    \Ndeen{-0.368} & \Ndeen{-0.365} & \Ndeen{-0.371} &
    % Complete curriculum
    %-.1184 & -.1110 & -.1090 & -.1041 & -.0972
    % Final curriculum
    \Ndeen{-0.363}
\\ \midrule

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%   ENGLISH -> CZECH
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\multirow{8}{*}{\rotatebox{90}{en-cs}}
& BLEU &
    % From random initialization
    \Bencs{21.06} & \Bencs{20.81} & \Bencs{20.93} & \Bencs{20.60} & \Bencs{20.10} & \Bencs{20.01} & \Bencs{19.52} & \Bencs{18.24} &
    % Direct finetuning
    \Bencs{19.25} & \Bencs{19.33} & \Bencs{19.42} & % \Bencs{18.13} &
    % Complete curriculum
    %\Bencs{19.26} & \Bencs{19.13} & \Bencs{19.15} & \Bencs{18.95} & \Bencs{18.96}
    % Final curriculum
    \Bencs{19.25}
\\
   &  &  % Comparing BLEU to the best scores
    % From random initialization
   \best{} & \fromBest{-0.25} & \fromBest{-0.13} & \fromBest{-0.46} & \fromBest{-0.96} & \fromBest{-1.05} & \fromBest{-1.54} & \fromBest{-2.82} &
    % Direct finetuning
    \compare{-1.81}{-0.27} & \compare{-1.73}{-0.68} & \compare{-1.64}{-0.68} &
    % Final curriculum
    \compare{-1.81}{-0.27}
\\
& chrF &
    % From random initialization
    \Cencs{.4893} & \Cencs{.4882} & \Cencs{.4899} & \Cencs{.4874} & \Cencs{.4831} & \Cencs{.4815} & \Cencs{.4782} & \Cencs{.4645} &
    % Direct finetuning
    \Cencs{.4766} & \Cencs{.4759} & \Cencs{.4782} & % \Cencs{.4662} &
    % Complete curriculum
    %\Cencs{.4770} & \Cencs{.4746} & \Cencs{.4741} & \Cencs{.4735} & \Cencs{.4728}
    % Final curriculum
    \Cencs{.4765}
\\
& METEOR &
    % From random initialization
    \Mencs{25.98} & \Mencs{25.79} & \Mencs{25.95} & \Mencs{25.82} & \Mencs{25.74} & \Mencs{25.73} & \Mencs{25.36} & \Mencs{24.57} &
    % Direct finetuning
    \Mencs{25.22} & \Mencs{25.16} & \Mencs{25.18} & % \Mencs{24.24} &
    % Complete curriculum
    %\Mencs{25.18} & \Mencs{25.05} & \Mencs{25.00} & \Mencs{24.90} & \Mencs{24.90}
    % Final curriculum
    \Mencs{25.08}
\\ \cdashlinelr{2-14}
& Noise sens. &
    % From random initialization
    \Nencs{-1.031} & \Nencs{-1.009} & \Nencs{-1.011} & \Nencs{-1.008} & \Nencs{-0.944} & \Nencs{-0.929} & \Nencs{-0.909} & \Nencs{-0.788} &
    % Direct finetuning
    \Nencs{-0.817} & \Nencs{-0.840} & \Nencs{-0.868} &
    % Complete curriculum
    % MISSING VALUES
    % Final curriculum
    \Nencs{-0.824}
\\
& MorphEval &
    % From random initialization
    \Rencs{83.86} & \Rencs{84.55} & \Rencs{83.73} & \Rencs{83.85} & \Rencs{84.27} & \Rencs{84.35} & \Rencs{84.68} & \Rencs{82.14} &
    % Direct finetuning
    \Rencs{84.68} & \Rencs{84.01} & \Rencs{81.85} &
    % Complete curriculum
    \Rencs{81.29}
%\\
%& Transliteration &
%    % From random initialization
%    \Tencs{4.91} & \Tencs{5.75} & \Tencs{4.83} & \Tencs{5.83} & \Tencs{5.30} & \Tencs{5.50} & \Tencs{4.74} &
%    % Direct finetuning
%    \Tencs{4.49} & \Tencs{4.99} & \Tencs{5.51} &
%    % Complete curriculum
%    \Tencs{4.99}
\\ \midrule

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%   ENGLISH -> TURKISH
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\multirow{4}{*}{\rotatebox{90}{en-tr}}
& BLEU &
    % From random initialization
    \Bentr{12.62} & \Bentr{13.10} & \Bentr{12.74} & \Bentr{12.81} & \Bentr{12.52} & \Bentr{12.33} & \Bentr{12.24} & \Bentr{12.37} &
    % Direct finetuning
    \Bentr{12.02} & \Bentr{12.25} & \Bentr{12.28} &
    % Complete curriculum
    \Bentr{11.56}
\\
   &  &  % Comparing BLEU to the best scores
    % From random initialization
    \fromBest{-0.48} & \best{} & \fromBest{-0.36} & \fromBest{-0.29} & \fromBest{-0.58} & \fromBest{-0.77} & \fromBest{-0.86} & \fromBest{-.0.73} &
    % Direct finetuning
    \compare{-1.08}{-0.22} & \compare{-0.85}{-0.08} & \compare{-0.82}{-0.53} &
    % Final curriculum
    \compare{-1.54}{-0.68}
\\
& chrF &
    % From random initialization
    \Centr{.4554} & \Centr{.4620} & \Centr{.4585} & \Centr{.4562} & \Centr{.4569} & \Centr{.4568} & \Centr{.4548} & \Centr{.4608} &
    % Direct finetuning
    \Centr{.4558} & \Centr{.4596} & \Centr{.4586} &
    % Complete curriculum
    \Centr{.4500}
\\ \cdashlinelr{2-14}

& Noise sens. &
    % From random initialization
    \Nentr{-0.916} & \Nentr{-0.912} & \Nentr{-0.896} & \Nentr{-0.869} & \Nentr{-0.849} & \Nentr{-0.828} & \Nentr{-0.794} & \Nentr{-0.615} &
    % Direct finetuning
    \Nentr{-0.659} & \Nentr{-0.660} & \Nentr{-0.658} &
    % Complete curriculum
    \Nentr{-0.676}
% \\ \midrule
% \multirow{4}{*}{\rotatebox{90}{en-ru}}
% & BLEU &
% \\
% & chrF &
% \\ \cdashlinelr{2-13}
% & Noise sens. &
% \\
% & Transliteration &

\\ \bottomrule

\end{tabular}}

